Unleashing the full potential of the North Sea -- Identifying key energy infrastructure synergies for 2030 and 2040

Policy efforts have primarily focused on expanding variable renewable energy sources (vRES) to meet carbon emission reduction targets. The integration of high shares of renewables into the energy system is central to both policy making and research, focusing on the need for balancing options between vRES and demand. In this work we analyze and compare three key integration measures: grid expansions, electricity storage, and the role of production, storage and transport of low-carbon hydrogen. We focus on their potential to reduce emissions and energy system costs, individually and in combination. We take the North Sea as an exemplary region with ambitious 2030-2040 targets for offshore wind developments. The projections on installed generation and grid capacities, along with demand estimates from the Ten Year Network Development Plan (TYNDP) 2022, serve as a starting point for our energy system model. This starting model can then be further expanded with the three integration measures. Our findings show that grid expansions across the North Sea are a no-regret measure lowering costs, emissions and required renewable. The production of hydrogen and its direct use in industry has a lower cost reduction potential and emission reduction potential, while hydrogen storage and transport have little to no additional value. In the short term (2030), electricity storage can help to reduce emissions, but it is not cost competitive. In the longer term (2040), storage can help to balance investments in vRES assets by providing additional flexibility to the system. Combining the three integration measures provides additional benefits. The highest emission reductions can be achieved by combining electricity storage with an expansion of the grid. The highest economic benefits can be achieved with a combination of grid expansions and hydrogen production for direct use in industry.

==> Tables/02_HydroInflows_Country.tex <==
\begin{table}
\centering
\caption{Hydro Inflows in TWh (aggregated per Country and per technology)}
\begin{tabular}{lr}
\toprule
{} &      0 \\
\midrule
(DE4, Hydro - Pump Storage Open Loop (Energy)) &   0.53 \\
(NO1, Hydro - Pump Storage Open Loop (Energy)) & 163.50 \\
(UK3, Hydro - Pump Storage Open Loop (Energy)) &   0.00 \\
(DE4, Hydro - Reservoir (Energy))              &   1.06 \\
(NO1, Hydro - Reservoir (Energy))              &   0.00 \\
(UK3, Hydro - Reservoir (Energy))              &   0.00 \\
\bottomrule
\end{tabular}
\end{table}


==> Tables/02_InstalledCapacities_RE_Country.tex <==
\begin{table}
\centering
\caption{Installed Capacities for onshore wind and PV in GW (aggregated per Country and per source)}
\begin{tabular}{lrrrr}
\toprule
{} &  PV (Our work) &  PV (TYNDP) &  Wind, onshore (Our work) &  Wind, onshore (TYNDP) \\
Country &                &             &                           &                        \\
\midrule
BE      &          10.40 &       10.40 &                      4.67 &                   4.67 \\
DE      &          96.14 &       96.14 &                     75.37 &                  75.37 \\
DK      &           6.47 &        6.47 &                      6.16 &                   6.16 \\
NL      &          27.26 &       27.26 &                      7.98 &                   7.98 \\
UK      &          23.41 &       23.41 &                     26.59 &                  26.59 \\
\bottomrule
\end{tabular}
\end{table}

